Making big steps in trajectories

We consider the solution of initial value problems within the context of hybrid systems and emphasise the use of high precision approximations (in software for exact real arithmetic). We propose a novel algorithm for the computation of trajectories up to the area where discontinuous jumps appear, applicable for holomorphic flow functions. Examples with a prototypical implementation illustrate that the algorithm might provide results with higher precision than well-known ODE solvers at a similar computation time.

==> eptcsdata.tex <==
\providecommand{\event}{X. Zheng and N. Zhong (Eds.)\\
Computability and Complexity in Analysis (CCA 2010)}
\providecommand{\volume}{24}
\providecommand{\anno}{2010}
\providecommand{\firstpage}{106}
\providecommand{\eid}{15}
\pdfoutput=1

